Pruning for Robust Concept Erasing in Diffusion Models

Despite the impressive capabilities of generating images, text-to-image diffusion models are susceptible to producing undesirable outputs such as NSFW content and copyrighted artworks. To address this issue, recent studies have focused on fine-tuning model parameters to erase problematic concepts. However, existing methods exhibit a major flaw in robustness, as fine-tuned models often reproduce the undesirable outputs when faced with cleverly crafted prompts. This reveals a fundamental limitation in the current approaches and may raise risks for the deployment of diffusion models in the open world. To address this gap, we locate the concept-correlated neurons and find that these neurons show high sensitivity to adversarial prompts, thus could be deactivated when erasing and reactivated again under attacks. To improve the robustness, we introduce a new pruning-based strategy for concept erasing. Our method selectively prunes critical parameters associated with the concepts targeted for removal, thereby reducing the sensitivity of concept-related neurons. Our method can be easily integrated with existing concept-erasing techniques, offering a robust improvement against adversarial inputs. Experimental results show a significant enhancement in our model's ability to resist adversarial inputs, achieving nearly a 40% improvement in erasing the NSFW content and a 30% improvement in erasing artwork style.

==> Figures/multi_erase.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.7\linewidth]{Images/multi-erase.pdf}
\caption{Visualization of multiple concept erasure. The input prompt is "a church and a garbage truck". Two rows are generated by different seeds. The first column are generated by the original model. The last three columns are generated by applying masks for erasing church, garbage truck, and both two.}
\label{fig:multi_erase}
\end{figure}


==> Tables/fid_compare.tex <==
% \begin{table}[htbp]
% \setlength\tabcolsep{5pt}
% \centering
% \caption{FID comparison.}
% \label{tab:nudity}
% \begin{tabular}{lcccccc}
% \toprule[1pt]
%  & SD & ESD & P-ESD \\  
% \midrule
% Erasing 
% \bottomrule[1pt]
% \end{tabular}
% \end{table}


% \begin{table}[htbp]
% \setlength\tabcolsep{5pt}
% \centering
% \caption{FID comparison.}
% \label{tab:fid_compare}
% \begin{tabular}{lccccccccc}
% \toprule[1pt]
%  & & SD & ESD & P-ESD \\  
% \midrule
% \multirow{2}{*}{\makecell{Erasing \\Nudity}} & FID-30k & 14.64 & 14.32 & 13.60 \\
% & CLIP & \\
% \midrule
% \multirow{2}{*}{\makecell{Erasing \\Style}} & FID-30k & 14.64 & 15.01 & 15.08 \\
% & CLIP & \\
% \bottomrule[1pt]
% \end{tabular}
% \end{table}



% \begin{table}[htbp]
% \setlength\tabcolsep{5pt}
% \centering
% \caption{FID comparison.}
% \label{tab:fid_compare}
% \begin{tabular}{lccccccccc}
% \toprule[1pt]
%  & SD & ESD & P-ESD \\  
% \midrule
% Erasing Nudity & \multirow{2}{*}{14.64} & 14.32 & 13.60 \\
% Erasing Style & & 15.01 & 15.08 \\
% \bottomrule[1pt]
% \end{tabular}
% \end{table}



% \begin{table}[htbp]
% \setlength\tabcolsep{5pt}
% \centering
% \caption{FID comparison.}
% \label{tab:fid_compare}
% \begin{tabular}{lccccccccc}
% \toprule[1pt]
%  & SD & ESD & P-ESD \\  
% \midrule
% Erasing Nudity & \multirow{2}{*}{14.64} & 14.32 & 13.60 \\
% Erasing Style & & 15.01 & 15.08 \\
% \bottomrule[1pt]
% \end{tabular}
% \end{table}



\begin{table}[htbp]
\setlength\tabcolsep{5pt}
\centering
\caption{FID comparison.}
\label{tab:fid_compare}
\begin{tabular}{lccccccccc}
\toprule[1pt]
 & SD & 14.64 \\  
\midrule
\multirow{2}{*}{nudity} & ESD & 14.32 \\
& P-ESD  & 13.60 \\
\midrule
\multirow{2}{*}{style} & ESD & 15.01 \\
& P-ESD &  15.08  \\
\bottomrule[1pt]
\end{tabular}
\end{table}



==> Tables/prune_compare.tex <==
% \begin{table}[htbp]
% \setlength\tabcolsep{5pt}
% \centering
% \caption{Compare different prune strategies.}
% \label{tab:prune_compare}
% \begin{tabular}{lccccccccc}
% \toprule[1pt]
% \multirow{2}{*}{Erasing Nudity} & \multicolumn{4}{c}{Nudity} \\
% \cmidrule{2-5} 
%  & w/o Prune & Pre-Prune & Post-Prune & Ours \\
% \midrule
% No-attack \\
% P4D \\
% UnlearnDiff \\
% \midrule[1pt]
% \multirow{2}{*}{Erasing Van Gogh} & \multicolumn{4}{c}{Van Gogh} \\
% \cmidrule{2-5} 
%  & w/o Prune & Pre-Prune & Post-Prune & Ours \\
% \midrule
% No-attack \\
% P4D \\
% UnlearnDiff \\
% \bottomrule[1pt]
% \end{tabular}
% \end{table}

\begin{table}[htbp]
\setlength\tabcolsep{5pt}
\centering
\caption{Compare different pruning strategies.}
\label{tab:prune_compare}
\begin{tabular}{lccccccccc}
\toprule[1pt]
 & & ESD & Pre-Prune & Post-Prune & P-ESD \\
\midrule
\multirow{3}{*}{\makecell{Erasing \\Nudity}} & No-attack & 10.53\% & 9.77\% & 13.53\% &  2.26\% \\
& UnlearnDiff & 36.84\% & 40.60\% & 33.83\% & 17.29\%\\
& P4D & 39.10\% & 30.83\%  & 39.85\% & 15.04\% \\
% \cmidrule{2-6}
% & FID \\
\midrule
\multirow{3}{*}{\makecell{Erasing \\Van Gogh}} & No-attack & 16.00\% & 12.00\% & 6.00\% & 0.00\%\\
& UnlearnDiff & 48.00\% & 46.00\% & 44.00\% & 12.00\%\\
& P4D & 44.00\%	& 36.00\% & 42.00\% & 16.00\%\\
% \cmidrule{2-6}
% & FID \\
\bottomrule[1pt]
\end{tabular}
\end{table}



==> Tables/storage_compare.tex <==

\begin{table}[htbp]
\setlength\tabcolsep{5pt}
\centering
\caption{Storage comparison.}
\label{tab:store_compare}
\begin{tabular}{lccccccccc}
\toprule[1pt]
 Method & Cross-attention & Non-cross-attention \\  
\midrule
Finetune-based & 175.9MB & 3.1GB \\
Ours  & 5.5MB & 98.4MB \\
\bottomrule[1pt]
\end{tabular}
\end{table}


